Dipole-Coupled Neutrissimo Explanations of the MiniBooNE Excess Including Constraints from MINERvA Data

We revisit models of heavy neutral leptons (neutrissimos) with transition magnetic moments as explanations of the $4.8\sigma$ excess of electron-like events at MiniBooNE. We perform a detailed Monte Carlo-based analysis to re-examine the preferred regions in the model parameter space to explain MiniBooNE, considering also potential contributions from oscillations due to an eV-scale sterile neutrino. We then derive robust constraints on the model using neutrino-electron elastic scattering data from MINERvA. We find that MINERvA rules out a large region of parameter space, but allowed solutions exist at the $2\sigma$ confidence level. A dedicated MINERvA analysis would likely be able to probe the entire region of preference of MiniBooNE in this model.

==> scratch.tex <==

\section{Interesting Papers} 

\begin{itemize}
    \item MiniBooNE Beam dump~\cite{Aguilar-Arevalo:2018wea}
    \item MiniBooNE latest~\cite{Aguilar-Arevalo:2020nvw}
    \item Minerva flux measurement with neutrino-electron scattering in LE mode~\cite{Park:2015eqa} and ME mode~\cite{Valencia:2019mkf}.
    \item CHARM-II neutrino-electron scattering final result~\cite{Vilain:1994qy} and useful references~\cite{DeWinter:1989zg,
Geiregat:1992zv,Allaby:1987bb}
    \item \emph{Arg\"uelles et al} on using neutrino-electron scattering to test upscattering-based explanations of MiniBooNE~\cite{Arguelles:2018mtc}.

    \item Measurement of the Inclusive Electron Neutrino Charged Current Cross
Section on Carbon with the T2K Near Detector (Jul 28, 2014)
\url{https://doi.org/10.1103/PhysRevLett.113.241803}
    \item Measurement of the charged-current electron (anti-)neutrino inclusive
cross-sections at the T2K off-axis near detector ND280 (Feb 27, 2020)
\url{https://doi.org/10.1007/JHEP10(2020)114}~\cite{Abe:2020vot}
    \item Measurement of the electron neutrino charged-current inclusive cross-section on carbon using the T2K near detector \url{https://spiral.imperial.ac.uk:8443/handle/10044/1/23284}

    
    
\end{itemize}



\section{Current electron-like excesses at neutrino experiments}

\begin{itemize}
    \item NOVA near detector. 
    \begin{itemize}
        \item Auxiliary measurement at ND for the oscillation analysis presented at~\href{https://indico.fnal.gov/event/43209/contributions/187840/attachments/130740/159597/NOvA-Oscilations-NEUTRINO2020.pdf}{A. Himmel's talk} at NEUTRINO2020.
        \item Same, but in the article with 2019 data~\cite{NOvA:2019cyt}
        \item $\nu_e$ CC inclusive cross section measurement (agreement with GENIE3.0.X.X, but less so with external MC predictions. See ~\href{https://zenodo.org/record/4155399#.YN3-qZNKiL4}{L. Cremonisi's talk} at NEUTRINO2020). See also ~\href{https://inspirehep.net/files/de0505656dd53c8c966da8531af0b55a}{M. Judah's thesis}, Fig. 5.17.
    \end{itemize}
    \item $\mu$BooNE NuMI events
    \begin{itemize}
        \item $\nu_e$CCQE measurement paper~\cite{MicroBooNE:2021ldh} (no energy spectrum shwown)
        \item Excess visible in \href{https://microboone.fnal.gov/wp-content/uploads/MICROBOONE-NOTE-1095-PUB.pdf}{public note} with energy spectrum in Fig. 53.
    \end{itemize}
    \item 
\end{itemize}




==> tikz_style.tex <==

\usetikzlibrary{trees}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}

\definecolor{kyelloworange}   {RGB}{255, 210,  110}
\definecolor{jblue}  {RGB}{20,50,100}
\definecolor{npurple}  {RGB} {153, 51, 204}
\definecolor{wred}   {RGB}{217,0,56}
\definecolor{white}   {RGB}{255,255,255}
  
\definecolor{korange}   {RGB}{235, 80,  43}
\definecolor{korange2}   {RGB}{245, 100,  63}
\definecolor{kyelloworange}   {RGB}{255, 210,  110}
\definecolor{kyelloworange2}   {RGB}{240, 170,  90}
\definecolor{kred}   {RGB}{204,  102, 153}
\definecolor{kpurple}   {RGB}{153,  61, 190}
\definecolor{kpurplelight}   {RGB}{213,  161, 230}

\tikzset{
	    gaugeboson/.style={decorate,decoration={snake, amplitude = 3pt, post length = 1 pt, pre length = 4 pt},draw=magenta},
	    fermion/.style={draw=black,postaction={decorate},decoration={markings,mark=at position .55}},
	    fermionin/.style={draw=black,postaction={decorate},decoration={markings,mark=at position .55 with {\arrow[draw=black]{<}}}},
	    fermionout/.style={draw=black,postaction={decorate},decoration={markings,mark=at position .55 with {\arrow[draw=black]{>}}}},
	    gluon/.style={decorate,draw=magenta,decoration={coil,amplitude = 6pt,segment length=8pt}},
	    connect/.style={draw=black,postaction={decorate},decoration={markings}}, %,mark=at position .55 with {\arrow[draw=red]{<}}}}
	    %QCD Corrections
	    gluon2/.style={decorate,draw=magenta,decoration={coil,amplitude = 3pt,segment length=4pt}},
	    gaugeboson2/.style={decorate,decoration={snake, amplitude = 3pt, segment length=6pt},draw=black}
	}
	
\tikzset{
	  photon/.style={decorate, decoration={snake}, draw=npurple,very thick},
	  boson/.style={decorate, decoration={snake}, draw=npurple,very thick},
	  electron/.style={draw=jblue,very thick, postaction={decorate},
	           decoration={markings,mark=at position .55 with {\arrow[draw=jblue]{>}}}
	  },
	  electron2/.style={draw=jblue,very thick, postaction={decorate},
	           decoration={markings,mark=at position .55 with {\arrow[draw=jblue]{<}}}
	  },
	  fermion/.style={draw=jblue,very thick, postaction={decorate},
	            decoration={markings,mark=at position .55 with {\arrow[draw=jblue]{}}}
	  },
	  gluon/.style={decorate, draw=korange,very thick, %kred
	    decoration={coil,amplitude=4pt, segment length=6pt}},
	  higgs/.style={draw=wred,very thick, postaction={decorate},
	           decoration={markings,mark=at position .55 with {\arrow[draw=wred]{>}}}
	  },
	  nothing/.style={draw=white,very thick}
}
